Characterisation of Laser Wakefield Acceleration Efficiency with Octave Spanning Near-IR Spectrum Measurements

We report on experimental measurements of energy transfer efficiencies in a GeV-class laser wakefield accelerator. Both the transfer of energy from the laser to the plasma wakefield, and from the plasma to the accelerated electron beam were diagnosed by simultaneous measurement of the deceleration of laser photons and the acceleration of electrons as a function of plasma length. The extraction efficiency, which we define as the ratio of the energy gained by the electron beam to the energy lost by the self-guided laser mode, was maximised at $19\pm3$\% by tuning of the plasma density and length. The additional information provided by the octave-spanning laser spectrum measurement allows for independent optimisation of the plasma efficiency terms, which is required for the key goal of improving the overall efficiency of laser wakefield accelerators.

==> Efficiency Measurement of Laser Wakefield Acceleration/authors.tex <==
\newcommand{\JAI}{The John Adams Institute for Accelerator Science, Imperial College London, London, SW7 2AZ, UK}

\newcommand{\GOLP}{GoLP/Instituto de Plasmas e Fus\~{a}o Nuclear, Instituto Superior T\'{e}cnico, U.L., Lisboa 1049-001, Portugal}

\newcommand{\CLF}{Central Laser Facility, STFC Rutherford Appleton Laboratory, Didcot OX11 0QX, UK}

\newcommand{\UCL}{Department of Physics and Astronomy, University College London, London WC1E 6BT, UK}

\newcommand{\LMU}{Fakult\"at f\"ur Physik, Ludwig-Maximilians-Universit\"at M\"unchen, D-85748 Garching, Germany}
\newcommand{\MPQ}{Max-Planck-Institut f\"ur Quantenoptik, Hans-Kopfermann-Str. 1, D-85748 Garching, Germany}

\newcommand{\DESY}{Deutsches Elektronen-Synchrotron DESY, Notkestr. 85, 22607 Hamburg, Germany}

\newcommand{\CI}{The Cockcroft Institute, Keckwick Lane, Daresbury, WA4 4AD, United Kingdom}

\newcommand{\LANCS}{Physics Department, Lancaster University, Lancaster LA1 4YB, United Kingdom}

\newcommand{\UMICH}{Center for Ultrafast Optical Science, University of Michigan, Ann Arbor, MI 48109-2099, USA}

\newcommand{\SUPA}{SUPA, Department of Physics, University of Strathclyde, Glasgow G4 0NG, UK}

\newcommand{\LLNL}{Lawrence Livermore National Laboratory (LLNL), P.O. Box 808, Livermore, California 94550, USA}

\newcommand{\DLS}{Diamond Light Source, Harwell Science and Innovation Campus, Fermi Avenue, Didcot OX11 0DE, UK}

\newcommand{\YORK}{York Plasma Institute, Department of Physics, University of York, York YO10 5DD, UK}

\newcommand{\ELI}{ELI-Beamlines, Institute of Physics, Academy of Sciences of the Czech Republic, 18221 Prague, Czech Republic}

\newcommand{\QUB}{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U.K.}

\newcommand{\LUND}{Department of Physics, Lund University, P.O. Box 118, S-22100, Lund, Sweden}
%%%%%%
%  author list: 
% alphabetical

\author{M.J.V.~Streeter}
\email{m.streeter@qub.ac.uk}
\affiliation{\CI}
\affiliation{\LANCS}
\affiliation{\JAI}
\affiliation{\QUB}

\author{Y.~Ma}
\affiliation{\UMICH}
\affiliation{\CI}
\affiliation{\LANCS}

\author{B.~Kettle}
\affiliation{\JAI}

\author{S.J.D.~Dann}
\affiliation{\CI}
\affiliation{\LANCS}


\author{E.~Gerstmayr}
\affiliation{\JAI}

\author{F.~Albert}
\affiliation{\LLNL}

\author{N.~Bourgeois}
\affiliation{\CLF}

\author{S.~Cipiccia}
\affiliation{\DLS}

\author{J.M.~Cole}
\affiliation{\JAI}

\author{I.G.~Gonz\'alez}
\affiliation{\LUND}

% \author{A.~Higginbotham}
% \affiliation{\YORK}

\author{A.E. ~Hussein}
\affiliation{\UMICH}

\author{D.A.~Jaroszynski}
\affiliation{\SUPA}
\affiliation{\CI}

\author{K.~Falk}
\affiliation{\ELI}

\author{K.~Krushelnick}
\affiliation{\UMICH}

\author{N.~Lemos}
\affiliation{\LLNL}

\author{N.C.~Lopes}
\affiliation{\JAI}
\affiliation{\GOLP}

\author{C.~Lumsdon}
\affiliation{\YORK}

\author{O.~Lundh}
\affiliation{\LUND}

\author{S.P.D.~Mangles}
\affiliation{\JAI}

\author{Z.~Najmudin}
\affiliation{\JAI}

\author{P.P.~Rajeev}
\affiliation{\CLF}

\author{M.~Shahzad}
\affiliation{\SUPA}
\affiliation{\CI}

\author{M.~Smid}
\affiliation{\ELI}

\author{R.~Sandberg}
\affiliation{\UMICH}

\author{R.~Spesyvtsev}
\affiliation{\SUPA}
\affiliation{\CI}

\author{D.R.~Symes}
\affiliation{\CLF}

\author{G.~Vieux}
\affiliation{\SUPA}
\affiliation{\CI}

% \author{J.~C.~Wood}
% \affiliation{\JAI}

\author{A.G.R.~Thomas}
\email{agrt@umich.edu}
\affiliation{\UMICH}
\affiliation{\CI}
\affiliation{\LANCS}


==> Efficiency Measurement of Laser Wakefield Acceleration/format.tex <==

\usepackage{graphicx}% Include figure files
% \graphicspath{{figures/}}
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{units}
\usepackage[colorlinks = true, linkcolor = blue,
            urlcolor  = blue,citecolor = blue,
            anchorcolor = blue]{hyperref}% add hypertext capabilities
\usepackage[noabbrev]{cleveref}
\usepackage[dvipsnames]{xcolor}
% \usepackage[colorinlistoftodos]{todonotes}


%\usepackage[mathlines]{lineno}% Enable numbering of text and display math
%\linenumbers\relax % Commence numbering lines

%\usepackage[showframe,%Uncomment any one of the following lines to test 
%%scale=0.7, marginratio={1:1, 2:3}, ignoreall,% default settings
%%text={7in,10in},centering,
%%margin=1.5in,
%%total={6.5in,8.75in}, top=1.2in, left=0.9in, includefoot,
%%height=10in,a5paper,hmargin={3cm,0.8in}
%]{geometry}

\renewcommand{\d}[2]{\frac{\mbox{d} #1}{\mbox{d} #2}} % for derivatives
\newcommand{\dd}[2]{\frac{\mbox{d}^2 #1}{\mbox{d} #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} % for partial derivatives
\newcommand{\avg}[1]{\left\langle #1 \right\rangle} % for average

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert} % for average

==> authors.tex <==
\newcommand{\JAI}{The John Adams Institute for Accelerator Science, Imperial College London, London, SW7 2AZ, UK}

\newcommand{\GOLP}{GoLP/Instituto de Plasmas e Fus\~{a}o Nuclear, Instituto Superior T\'{e}cnico, U.L., Lisboa 1049-001, Portugal}

\newcommand{\CLF}{Central Laser Facility, STFC Rutherford Appleton Laboratory, Didcot OX11 0QX, UK}

\newcommand{\UCL}{Department of Physics and Astronomy, University College London, London WC1E 6BT, UK}

\newcommand{\LMU}{Fakult\"at f\"ur Physik, Ludwig-Maximilians-Universit\"at M\"unchen, D-85748 Garching, Germany}
\newcommand{\MPQ}{Max-Planck-Institut f\"ur Quantenoptik, Hans-Kopfermann-Str. 1, D-85748 Garching, Germany}

\newcommand{\DESY}{Deutsches Elektronen-Synchrotron DESY, Notkestr. 85, 22607 Hamburg, Germany}

\newcommand{\CI}{The Cockcroft Institute, Keckwick Lane, Daresbury, WA4 4AD, United Kingdom}

\newcommand{\LANCS}{Physics Department, Lancaster University, Lancaster LA1 4YB, United Kingdom}

\newcommand{\UMICH}{Center for Ultrafast Optical Science, University of Michigan, Ann Arbor, MI 48109-2099, USA}

\newcommand{\SUPA}{SUPA, Department of Physics, University of Strathclyde, Glasgow G4 0NG, UK}

\newcommand{\LLNL}{Lawrence Livermore National Laboratory (LLNL), P.O. Box 808, Livermore, California 94550, USA}

\newcommand{\DLS}{Diamond Light Source, Harwell Science and Innovation Campus, Fermi Avenue, Didcot OX11 0DE, UK}

\newcommand{\YORK}{York Plasma Institute, Department of Physics, University of York, York YO10 5DD, UK}

\newcommand{\ELI}{ELI-Beamlines, Institute of Physics, Academy of Sciences of the Czech Republic, 18221 Prague, Czech Republic}

\newcommand{\QUB}{School of Maths and Physics, Queen's University Belfast, University Road, Belfast, N. Ireland, U.K.}

\newcommand{\LUND}{Department of Physics, Lund University, P.O. Box 118, S-22100, Lund, Sweden}
%%%%%%
%  author list: 
% alphabetical

\author{M.J.V.~Streeter}
\email{m.streeter@qub.ac.uk}
\affiliation{\CI}
\affiliation{\LANCS}
\affiliation{\JAI}
\affiliation{\QUB}

\author{Y.~Ma}
\affiliation{\UMICH}
\affiliation{\CI}
\affiliation{\LANCS}

\author{B.~Kettle}
\affiliation{\JAI}

\author{S.J.D.~Dann}
\affiliation{\CI}
\affiliation{\LANCS}


\author{E.~Gerstmayr}
\affiliation{\JAI}

\author{F.~Albert}
\affiliation{\LLNL}

\author{N.~Bourgeois}
\affiliation{\CLF}

\author{S.~Cipiccia}
\affiliation{\DLS}

\author{J.M.~Cole}
\affiliation{\JAI}

\author{I.G.~Gonz\'alez}
\affiliation{\LUND}

% \author{A.~Higginbotham}
% \affiliation{\YORK}

\author{A.E. ~Hussein}
\affiliation{\UMICH}

\author{D.A.~Jaroszynski}
\affiliation{\SUPA}
\affiliation{\CI}

\author{K.~Falk}
\affiliation{\ELI}

\author{K.~Krushelnick}
\affiliation{\UMICH}

\author{N.~Lemos}
\affiliation{\LLNL}

\author{N.C.~Lopes}
\affiliation{\JAI}
\affiliation{\GOLP}

\author{C.~Lumsdon}
\affiliation{\YORK}

\author{O.~Lundh}
\affiliation{\LUND}

\author{S.P.D.~Mangles}
\affiliation{\JAI}

\author{Z.~Najmudin}
\affiliation{\JAI}

\author{P.P.~Rajeev}
\affiliation{\CLF}

\author{M.~Shahzad}
\affiliation{\SUPA}
\affiliation{\CI}

\author{M.~Smid}
\affiliation{\ELI}

\author{R.~Sandberg}
\affiliation{\UMICH}

\author{R.~Spesyvtsev}
\affiliation{\SUPA}
\affiliation{\CI}

\author{D.R.~Symes}
\affiliation{\CLF}

\author{G.~Vieux}
\affiliation{\SUPA}
\affiliation{\CI}

% \author{J.~C.~Wood}
% \affiliation{\JAI}

\author{A.G.R.~Thomas}
\email{agrt@umich.edu}
\affiliation{\UMICH}
\affiliation{\CI}
\affiliation{\LANCS}


==> format.tex <==

\usepackage{graphicx}% Include figure files
% \graphicspath{{figures/}}
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{units}
\usepackage[colorlinks = true, linkcolor = blue,
            urlcolor  = blue,citecolor = blue,
            anchorcolor = blue]{hyperref}% add hypertext capabilities
\usepackage[noabbrev]{cleveref}
\usepackage[dvipsnames]{xcolor}
% \usepackage[colorinlistoftodos]{todonotes}


%\usepackage[mathlines]{lineno}% Enable numbering of text and display math
%\linenumbers\relax % Commence numbering lines

%\usepackage[showframe,%Uncomment any one of the following lines to test 
%%scale=0.7, marginratio={1:1, 2:3}, ignoreall,% default settings
%%text={7in,10in},centering,
%%margin=1.5in,
%%total={6.5in,8.75in}, top=1.2in, left=0.9in, includefoot,
%%height=10in,a5paper,hmargin={3cm,0.8in}
%]{geometry}

\renewcommand{\d}[2]{\frac{\mbox{d} #1}{\mbox{d} #2}} % for derivatives
\newcommand{\dd}[2]{\frac{\mbox{d}^2 #1}{\mbox{d} #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} % for partial derivatives
\newcommand{\avg}[1]{\left\langle #1 \right\rangle} % for average

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert} % for average
